MegaCOIN: Enhancing Medium-Grained Color Perception for Vision-Language Models

In vision-language models (VLMs), the ability to perceive and interpret color and physical environment is crucial for achieving contextually accurate understanding and interaction. However, despite advances in multimodal modeling, there remains a significant lack of specialized datasets that rigorously evaluate a model's capacity to discern subtle color variations and spatial context -- critical elements for situational comprehension and reliable deployment across real-world applications. Toward that goal, we curate MegaCOIN, a high-quality, human-labeled dataset based on \emph{real} images with various contextual attributes. MegaCOIN consists of two parts: MegaCOIN-Instruct, which serves as a supervised fine-tuning (SFT) dataset for VLMs; and MegaCOIN-Bench, an annotated test set that can be used as a stand-alone QA dataset. MegaCOIN~provides three annotated features for 220,000 real images: foreground color, background color, and description of an object's physical environment, constituting 660k human annotations. In addition, MegaCOIN can be applied to benchmark domain generalization (DG) algorithms. We explore benchmarking DG methods in the linear probing setup for VLM and show some new insights. Last but not least, we show that VLMs, including GPT-4o, have subpar color recognition capabilities, and fine-tuning with MegaCOIN can result in improved performance on visual evaluation tasks. In certain cases, MegaCOIN fine-tuned small-scale opensource models such as LLaVA and Bunny can outperform closed-source GPT-4o. We hope the utilities of MegaCOIN can shed light on the directions VLMs can improve and provide a more complex platform for domain generalization algorithms.

==> tables/july_clip_lienar_probe.tex <==

\begin{table*}[ht]
    \centering
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{cccccccc}
\toprule
Dataset & CORAL & CausIRL\_MMD & EQRM & ERM & GroupDRO & IRM & MMD \\
\midrule
Cifar10BGD & \textbf{97.78(0.10)} & 97.69(0.17) & 97.74(0.12) & 97.72(0.17) & 97.72(0.13) & 97.32(0.72) & 97.76(0.11) \\
% \hline
Cifar10BGDmerge & 97.71(0.17) & 97.72(0.12) & 97.69(0.13) & 97.67(0.14) & 97.74(0.11) & 96.98(0.96) & \textbf{97.76(0.12)} \\
% \hline
Cifar10ENV & 97.59(0.09) & 97.59(0.09) & 97.57(0.12) & 97.62(0.13) & 97.52(0.13) & $97.58(0.00)^*$ & \textbf{$97.75(0.00)^{*}$} \\
% \hline
Cifar10FGD & 97.64(0.10) & 97.62(0.13) & 97.60(0.08) & \textbf{97.65(0.11)} & 97.54(0.10) & 97.13(0.65) & 97.61(0.07) \\
% \hline
Cifar10FGDmerge & 97.64(0.10) & 97.63(0.12) & 97.62(0.13) & \textbf{97.66(0.12)} & 97.60(0.14) & 97.10(0.81) & \textbf{97.66(0.10)} \\
% \hline
TinyImagenetBGD & 80.36(0.40) & 80.43(0.31) & 80.29(0.33) & \textbf{80.64(0.33)} & 79.81(0.45) & 74.27(5.55) & 80.36(0.34) \\
% \hline
TinyImagenetBGDmerge & 80.73(0.26) & 80.76(0.46) & 80.62(0.29) & \textbf{80.78(0.24)} & 80.19(0.63) & 75.05(6.39) & 80.77(0.29) \\
% \hline
TinyImagenetENV & \textbf{79.79(0.31)} & 79.53(0.29) & 79.59(0.36) & 79.60(0.36) & 78.69(0.78) & - & - \\
% \hline
TinyImagenetFGD & 80.32(0.30) & \textbf{80.41(0.33)} & 80.19(0.38) & 80.24(0.42) & 79.58(0.47) & 73.84(6.00) & 80.23(0.31) \\
% \hline
TinyImagenetFGDmerge & 80.60(0.27) & 80.53(0.34) & 80.41(0.44) & 80.56(0.26) & 80.09(0.39) & 75.26(6.61) & \textbf{80.62(0.30)} \\
\hline
Average &&&&&&& \\
\bottomrule
\end{tabular}
\end{adjustbox}
    \caption{resent results}
    \label{tab:my_label}
\end{table*}

==> tables/statistic_color_merge.tex <==
\begin{table*}
\label{tab:color_count}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lcccccccccc}
\toprule
Dataset & Split & black & blue & brown & gray & green & others & red & white & yellow \\
% Dataset & Set &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{2}{*}{C10FGDmerge} & train & 7414 & 2862 & 12910 & 11085 & 2495 & 190 & 3158 & 7171 & 2715\\
 & test & 1504 & 573 & 2824 & 1889 & 447 & 42 & 607 & 1638 & 476  \\
\cmidrule{1-11}
\multirow[c]{2}{*}{TIFGDmerge} & train & 17144 & 4891 & 22842 & 21286 & 5715 & 5176 & 7860 & 4739 & 10347 \\
 & test & 1638 & 492 & 2271 & 1993 & 578 & 536 & 846 & 729 & 917 \\
\cmidrule{1-11}
\multirow[c]{2}{*}{C10BGDmerge} & train & 4830 & 8102 & 6995 & 13129 & 10592 & 532 & 989 & 3408 & 1423 \\
 & test & 723 & 1649 & 1460 & 2470 & 2314 & 227 & 187  & 759 & 211 \\
 \cmidrule{1-11}
\multirow[c]{2}{*}{TIBGDmerge}  & train & 9172 & 11169 & 15754 & 30844 & 17064 & 3395 & 2304 & 5864 & 4434\\
 & test & 894 & 1113 & 1500 & 3079 & 1754 & 227 & 248 & 784 & 401 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Statistics of \coin (Merged Foreground and Merged Background) }
\end{table*}

==> tables/unused_tables.tex <==


\begin{table}[]
    \centering
    \caption{Dataset Statistics-Color}
    \begin{tabular}{ccccccccccccc}
        \toprule
        Color & red & green & blue & black & white & brown & yellow & orange & pink & gray & violet & others \\\midrule
        CIFAR10-train & & & & & & & & & & & & \\
        CIFAR10-test & & & & & & & & & & & & \\
        Tiny-Imagenet-train & & & & & & & & & & & & \\
        Tiny-Imagenetest & & & & & & & & & & & & \\
        ImageNet & & & & & & & & & & & & \\\bottomrule
    \end{tabular}
    
    \label{tab:statistics_color}
\end{table}

\begin{table}[]
    \centering
    \caption{Dataset Statistics-Environment}
    \begin{tabular}{ccccccc}
        \toprule
         & Water & Land & Sky & Indoor & Plain & Others \\\midrule
        CIFAR10-train & & & & & & \\
        CIFAR10-test & & & & & & \\
        Tiny-Imagenet-train & & & & & & \\
        Tiny-Imagenet-test & & & & & & \\
        ImageNet & & & & & & \\\bottomrule
    \end{tabular}
    
    \label{tab:statistics_env}
\end{table}



==> tables/worst_group_bgd.tex <==
\begin{table}[h]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccccccccc}
\toprule
Dataset & CORAL & EQRM & ERM & GroupDRO & MMD & SelfReg & VREx \\ \midrule
C10BGD$\times$FGD & 95.95 & 95.00 & 96.37 & 96.44 & 96.76 & 93.81 & 96.45 \\ %\hline
C10BGD$\times$ENV & 96.37 & 96.04 & 96.17 & 96.28 & 96.42 & 95.98 & 95.88 \\ %\hline
TIBGD$\times$FGD & 77.52 & 76.76 & 76.95 & 75.90 & 75.14 & 76.48 & 71.90 \\ %\hline
TIBGD$\times$ENV & 77.53 & 77.70 & 78.02 & 76.26 & 77.72 & 77.21 & 75.26 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Worst Group Performance of Algorithms Trained on BGD and Evaluated on FGD and ENV. }
\label{tab:worst_bgd}
\end{table}

==> tables/worst_group_env.tex <==
\begin{table}[h]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|cccccccc}\toprule
Dataset & CORAL & EQRM & ERM & GroupDRO & MMD & SelfReg & VREx \\ \midrule
C10ENV$\times$FGD & 95.71 & 95.71 & 95.95 & 96.32 & 96.43 & 94.52 & 94.52 \\ %\hline
C10ENV$\times$BGD & 94.26 & 94.04 & 94.04 & 93.62 & 93.40 & 94.63 & 94.36 \\ %\hline
TIENV$\times$FGD & 76.12 & 75.91 & 76.06 & 73.24 & 75.97 & 75.56 & 74.87 \\ %\hline
TIENV$\times$BGD & 75.56 & 75.89 & 76.85 & 74.03 & 75.56 & 75.00 & 73.79 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Worst Group Performance of Algorithms Trained on ENV and Evaluated on FGD and BGD. }
\label{tab:worst_env}
\end{table}

==> tables/worst_group_fgd.tex <==
\begin{table}[h]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccccccccc}
\toprule
Trained on FGD & CORAL & EQRM & ERM & GroupDRO & MMD & SelfReg & VREx \\ \midrule
C10FGD$\times$BGD & 94.47 & 94.36 & 93.19 & 94.36 & 94.47 & 93.72 & 94.04 \\ %\hline
C10FGD$\times$ENV & 95.95 & 95.94 & 96.27 & 95.46 & 95.81 & 96.07 & 95.41 \\ %\hline
TIFGD$\times$BGD & 74.19 & 73.63 & 74.52 & 73.31 & 73.79 & 73.79 & 69.76 \\ %\hline
TIFGD$\times$ENV & 77.87 & 77.43 & 77.34 & 76.43 & 77.41 & 77.23 & 74.47 \\ \hline
Average & & & & & & & \\
\midrule
C10BGD $\times$ FGD &&&&&&&& \\
\midrule
Average &&&&&&&& \\
\end{tabular}
\end{adjustbox}
\caption{Worst Group Performance of Algorithms Trained on FGD and Evaluated on BGD and ENV. }
\label{tab:worst_fgd}
\end{table}
